Quasi-symmetry protected topology in a semi-metal

The crystal symmetry of a material dictates the type of topological band structures it may host, and therefore symmetry is the guiding principle to find topological materials. Here we introduce an alternative guiding principle, which we call 'quasi-symmetry'. This is the situation where a Hamiltonian has an exact symmetry at lower-order that is broken by higher-order perturbation terms. This enforces finite but parametrically small gaps at some low-symmetry points in momentum space. Untethered from the restraints of symmetry, quasi-symmetries eliminate the need for fine-tuning as they enforce that sources of large Berry curvature will occur at arbitrary chemical potentials. We demonstrate that a quasi-symmetry in the semi-metal CoSi stabilizes gaps below 2 meV over a large near-degenerate plane that can be measured in the quantum oscillation spectrum. The application of in-plane strain breaks the crystal symmetry and gaps the degenerate point, observable by new magnetic breakdown orbits. The quasi-symmetry, however, does not depend on spatial symmetries and hence transmission remains fully coherent. These results demonstrate a class of topological materials with increased resilience to perturbations such as strain-induced crystalline symmetry breaking, which may lead to robust topological applications as well as unexpected topology beyond the usual space group classifications.

==> preamble.tex <==
%\pdfoutput=1
\setlength{\intextsep}{10pt}
\setlength{\textfloatsep}{5pt}

%adjust height of rows in a table
\setlength\extrarowheight{2.5pt}

\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}p{#1}}

%% ultimate commands
	
	% align environment
			\newcommand{\e}[1]{\begin{align}{#1}\end{align}}	
	
		
	% fraction
		\newcommand{\f}[2]{\frac{#1}{#2}}
		\newcommand{\tf}[2]{\tfrac{#1}{#2}}
		
	% partial differentiation
		\newcommand{\p}[2]{\frac{\partial #1}{\partial #2}}
		\newcommand{\pf}[3]{\frac{\partial #1}{\partial #2}\bigg|_{#3}}
		\newcommand{\pa}[1]{\partial_{#1}}
		
	% label equations/sections
		\newcommand{\la}[1]{\label{#1}}

	% refer to equation, section, figure, appendix
		\newcommand{\q}[1]{Eq.\ (\ref{#1})}
		\newcommand{\qq}[2]{Eqs.\ (\ref{#1})-(\ref{#2})}
		\newcommand{\s}[1]{Sec.\ \ref{#1}}
		\newcommand{\fig}[1]{Fig.\ \ref{#1}}		
		\newcommand{\app}[1]{App.\ \ref{#1}}				
		\newcommand{\tab}[1]{Tab.\ \ref{#1}}
		\newcommand{\ocite}[1]{Ref.\ \onlinecite{#1}}
		\newcommand{\cf}[1]{[cf.\ Eq.\ (\ref{#1})]}
	
				
	% brackets
		\newcommand{\brac}[1]{\left(\;#1\;\right)}
		\newcommand{\sq}[1]{\left[\;#1\;\right]}
		\newcommand{\cu}[1]{\left\{\;#1\;\right\}}

	% insert words in equation environment

		\newcommand{\iwith}{\ins{with}}
		\newcommand{\where}{\ins{where}}		
		\newcommand{\iand}{\ins{and}}
		\newcommand{\ior}{\ins{or}}
		\newcommand{\ifor}{\ins{for}}
		\newcommand{\st}{\ins{s.t.}}
		
	% sign functions
		\newcommand{\sgn}{\text{sgn}}

	% equal, approximate, proportional signs, limits
		\newcommand{\eq}{=&\;}
		\newcommand{\condeq}[1]{\as \substack{\sma{#1}\\=}\as}
		\newcommand{\condprop}[1]{\as \substack{\sma{#1}\\ \propto}\as}
		\newcommand{\limit}[1]{\substack{\text{lim}\\#1}\as}		
		\newcommand{\appr}{\approx &\;}
		\newcommand{\prop}{\propto&\;}
		\newcommand{\define}{\as\substack{\text{def}\\ \iff}\as}					
	
	% mathbb symbols
		\newcommand{\F}{\mathbb{F}}
		\newcommand{\R}{\mathbb{R}}
		\newcommand{\Z}{\mathbb{Z}}
		\newcommand{\I}{\mathbb{I}}
		\newcommand{\C}{\mathbb{C}}
		\newcommand{\N}{\mathbb{N}}		
		\newcommand{\Q}{\mathbb{Q}}				
		\newcommand{\bbs}{\mathbb{S}}
		\newcommand{\bbt}{\mathbb{T}}

		
% for review
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}

% exponential 
\newcommand{\ex}{\text{exp}}
\newcommand{\pexp}{\overline{\text{exp}}}
		
		
% plane wave
	\newcommand{\eikr}{e^{i\bk \cdot \br}}
	\newcommand{\eikR}{e^{i\bk \cdot \bR}}
	\newcommand{\emikr}{e^{-i\bk \cdot \br}}
	\newcommand{\emikR}{e^{-i\bk \cdot \bR}}	

% divergence,curl,laplacian
\newcommand{\na}{\nabla}
\newcommand{\nai}{\nabla_i}
\newcommand{\naj}{\nabla_j}
\newcommand{\nak}{\nabla_k}
\newcommand{\nal}{\nabla_l}
\newcommand{\diverge}{\nabla \cdot}
\newcommand{\curl}{\nabla \times}
\newcommand{\lap}{\nabla^2}
\newcommand{\nabr}{\nabla_{\boldsymbol{r}}}
\newcommand{\nabk}{\nabla_{\boldsymbol{k}}}
\newcommand{\nabkp}{\nabla_{\boldsymbol{k}'}}

%fundamental constants
\newcommand{\bohr}{\mu_{\sma{B}}}
\newcommand{\gfac}{g_{\sma{0}}}
\newcommand{\lmt}{l^{\mt}}
\newcommand{\lmf}{l^{\text{-}4}}
\newcommand{\lmo}{l^{\mo}}




% specific to geometric_orbital
\newcommand{\om}{orbital moment }
\newcommand{\omm}{orbital moment}
\newcommand{\zf}{Zilberman-Fischbeck }
\newcommand{\checkgp}{\check{g}^{\sma{\perp}}}
\newcommand{\btperp}{$BT_{\sma{\perp}}$}
\newcommand{\bise}{Bi$_2$Se$_3$}



% c creation operators

\newcommand{\cdagk}{\dg{c}_{\bk}}
\newcommand{\ck}{\pdg{c}_{\bk}}
\newcommand{\cdagksig}{\dg{c}_{\bk,\sigma}}
\newcommand{\cksig}{\pdg{c}_{\bk,\sigma}}
\newcommand{\cdagkup}{c^\dagger_{\boldsymbol{k}\uparrow}}
\newcommand{\cdagkdo}{c^\dagger_{\boldsymbol{k}\downarrow}}
\newcommand{\ckup}{\pdg{c}_{\boldsymbol{k} \uparrow}}
\newcommand{\ckdo}{\pdg{c}_{\boldsymbol{k} \downarrow}}

\newcommand{\cdag}[1]{c^{\scriptscriptstyle{\dagger}}_{\scriptstyle{#1}}}
\newcommand{\cnod}[1]{c_{\scriptstyle{#1}}}


\newcommand{\cdj}{c^{\scriptscriptstyle{\dagger}}_{\scriptstyle{j \sigma}}}
\newcommand{\cnj}{c_{\scriptstyle{j' \sigma'}}}


% f creation operator

\newcommand{\fsig}{\pdg{f}_{\sigma}}
\newcommand{\fdagsig}{\dg{f}_{\sigma}}
\newcommand{\fup}{\pdg{f}_{\uparrow}}
\newcommand{\fdagup}{\dg{f}_{\uparrow}}
\newcommand{\fdo}{\pdg{f}_{\downarrow}}
\newcommand{\fdagdo}{\dg{f}_{\downarrow}}


%levi Cevita
\newcommand{\levi}[1]{\epsilon_{#1}}


%spin symbols
\newcommand\nup{\hat{n}_{f\uparrow}}
\newcommand\ndo{\hat{n}_{f\downarrow}}
\newcommand\avenup{{n}_{f\uparrow}}
\newcommand\avendo{{n}_{f\downarrow} }

% energies with varepsilon
\newcommand{\var}{\varepsilon}
%\newcommand{\var}[1]{\varepsilon_{#1}}
\newcommand{\efu}{\varepsilon_{\scriptscriptstyle{F}}^{\scriptscriptstyle{\uparrow}}}
\newcommand{\efd}{\varepsilon_{\scriptscriptstyle{F}}^{\scriptscriptstyle{\downarrow}}}
\newcommand{\ef}{\varepsilon_{\scriptscriptstyle{f}}}
\newcommand{\EF}{E_{\scriptscriptstyle{F}}}
\newcommand{\ek}{\varepsilon_{\boldsymbol{k}}}
\newcommand{\eF}{\varepsilon_{\scriptscriptstyle{F}}}
\newcommand{\enk}{\varepsilon_{n,\bk}}




% space

\newcommand\as{\;\;\;\;}
\newcommand\ass{\;\;\;\;\;\;\;\;}


\newcommand\Wline[2]{ \pdg{\W}_{\sma{#1 \leftarrow #2}}}


%hat operators

\newcommand{\hn}{\hat{n}}
\newcommand{\hp}{\hat{p}}
\newcommand{\hq}{\hat{q}}
\newcommand{\hA}{\hat{A}}
\newcommand{\hB}{\hat{B}}
\newcommand{\hC}{\hat{C}}
\newcommand{\hD}{\hat{D}}
\newcommand{\hE}{\hat{E}}
\newcommand{\hF}{\hat{F}}
\newcommand{\hG}{\hat{G}}
\newcommand{\hH}{\hat{H}}
\newcommand{\hJ}{\hat{J}}
\newcommand{\hK}{\hat{K}}
\newcommand{\hN}{\hat{N}}
\newcommand{\hO}{\hat{O}}
\newcommand{\hPi}{\hat{{\Pi}}}
\newcommand{\hpsi}{\hat{{\psi}}}
\newcommand{\hphi}{\hat{{\phi}}}
\newcommand{\hrho}{\hat{{\rho}}}
\newcommand{\hsigma}{\hat{{\sigma}}}
	%hatted operators with dagger
	\newcommand{\dhpsi}{\dg{\hat{{\psi}}}}
	\newcommand{\dhphi}{\dg{\hat{{\phi}}}}


%hatted bold symbols
\newcommand{\hbp}{\hat{\bp}}
\newcommand{\hbr}{\hat{\br}}
\newcommand{\hbv}{\hat{\bv}}
\newcommand{\hbx}{\hat{\bx}}
\newcommand{\bhp}{\boldsymbol{\hat{p}}}
\newcommand{\hbA}{\hat{\bA}}
\newcommand{\hbB}{\hat{\bB}}
\newcommand{\hbJ}{\hat{\bJ}}
\newcommand{\hbP}{\hat{\bP}}
\newcommand{\hbpi}{\hat{\boldsymbol{\pi}}}
\newcommand{\hbPi}{\hat{\boldsymbol{\Pi}}}


%bold symbols

\newcommand{\ba}{\boldsymbol{a}}
\newcommand{\bb}{\boldsymbol{b}}
\newcommand{\bc}{\boldsymbol{c}}
\newcommand{\bd}{\boldsymbol{d}}
\newcommand{\be}{\boldsymbol{e}}
\newcommand{\bff}{\boldsymbol{f}}
\newcommand{\bg}{\boldsymbol{g}}
\newcommand{\bh}{\boldsymbol{h}}
\newcommand{\bi}{\boldsymbol{i}}
\newcommand{\bj}{\boldsymbol{j}}
\newcommand{\bk}{\boldsymbol{k}}
\newcommand{\bkp}{\boldsymbol{k}_{\sma{\perp}}}
\newcommand{\bkpar}{\bk_{\parallel}}
\newcommand{\bkone}{\boldsymbol{k_1}}
\newcommand{\bktwo}{\boldsymbol{k_2}}
\newcommand{\bn}{\boldsymbol{n}}
\newcommand{\bp}{\boldsymbol{p}}
\newcommand{\bq}{\boldsymbol{q}}
\newcommand{\br}{\boldsymbol{r}}
\newcommand{\brp}{\boldsymbol{r}_{\sma{\perp}}}
\newcommand{\bs}{\boldsymbol{s}}
\newcommand{\bt}{\boldsymbol{t}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bz}{\boldsymbol{z}}
\newcommand{\bA}{\boldsymbol{A}}
\newcommand{\bB}{\boldsymbol{B}}
\newcommand{\bC}{\boldsymbol{C}}
\newcommand{\bD}{\boldsymbol{D}}
\newcommand{\bE}{\boldsymbol{E}}
\newcommand{\bF}{\boldsymbol{F}}
\newcommand{\bG}{\boldsymbol{G}}
\newcommand{\bH}{\boldsymbol{H}}
\newcommand{\bI}{\boldsymbol{I}}
\newcommand{\bJ}{\boldsymbol{J}}
\newcommand{\bK}{\boldsymbol{K}}
\newcommand{\bM}{\boldsymbol{M}}
\newcommand{\bL}{\boldsymbol{L}}
\newcommand{\bO}{\boldsymbol{O}}
\newcommand{\bP}{\boldsymbol{P}}
\newcommand{\bQ}{\boldsymbol{Q}}
\newcommand{\bR}{\boldsymbol{R}}
\newcommand{\bS}{\boldsymbol{S}}
\newcommand{\bV}{\boldsymbol{V}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bY}{\boldsymbol{Y}}
\newcommand{\bZ}{\boldsymbol{Z}}
\newcommand{\bze}{\boldsymbol{0}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\bPi}{\boldsymbol{\Pi}}
\newcommand{\bcalf}{\boldsymbol{\calf}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\bkappa}{\boldsymbol{\kappa}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bomega}{\boldsymbol{\omega}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\btau}{\boldsymbol{\tau}}
\newcommand{\bvarphi}{\boldsymbol{\varphi}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bvarpi}{\boldsymbol{\varpi}}
\newcommand{\bdeltapar}{\boldsymbol{\delta}_{\sma{\parallel}}}
\newcommand{\bna}{\boldsymbol{\nabla}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}



%\mathfrak
\newcommand{\frake}{\mathfrak{e}}
\newcommand{\frako}{\mathfrak{o}}
\newcommand{\frakt}{\mathfrak{t}}
\newcommand{\fraks}{\mathfrak{s}}
\newcommand{\frakr}{\mathfrak{r}}
\newcommand{\mx}{\mathfrak{X}}
\newcommand{\mxx}{\mathfrak{X}^x}
\newcommand{\mxy}{\mathfrak{X}^y}
\newcommand{\bmx}{\bar{M}_x}


\newcommand{\orb}{\boldsymbol{\mathfrak{A}}}
\newcommand{\lutt}{\boldsymbol{\mathfrak{L}}}



%tilde
\newcommand{\tbPi}{\tilde{\bPi}}
\newcommand{\tPi}{\tilde{\Pi}}
\newcommand{\txi}{\tilde{\xi}}
\newcommand{\tbv}{\tilde{\bv}}
\newcommand{\tv}{\tilde{v}}
\newcommand{\tbmx}{\tilde{\bmx}}
\newcommand{\tmxx}{\tilde{\mx}^x}
\newcommand{\tmxy}{\tilde{\mx}^y}
\newcommand{\tmx}{\tilde{\mx}}
\newcommand{\tH}{\tilde{H}}
\newcommand{\tbsigma}{\tilde{\bsigma}}
\newcommand{\tsigma}{\tilde{\sigma}}
\newcommand{\tilu}[1]{\tilde{u}_{#1}}
\newcommand\tilX{\tilde{X}}
\newcommand\tilZ{\tilde{Z}}
\newcommand\tilGamma{\tilde{\Gamma}}
\newcommand\tilU{\tilde{U}}

%calligraphic
\newcommand{\calL}{{\cal L}}
\newcommand{\W}{{\cal W}}
\newcommand{\A}{{\cal A}}


% equal signs
\newcommand\kzeq{\;\stackrel{\mathclap{\normalfont\mbox{$\sma{\bar{k}_z}$}}}{=}\;}

%breve 
\newcommand{\breveg}{\breve{g}}


% symmetry operators
\newcommand{\inv}{\mathfrak{i}}
\newcommand{\mir}{\mathfrak{r}}
\newcommand\glide{\mathfrak{g}}
\newcommand\rot{\mathfrak{c}}
\newcommand\scr{\mathfrak{s}}
\newcommand\tra{\mathfrak{t}}


\newcommand{\calti}{{\cal T}_{\sma{\cal I}}}
\newcommand{\gdel}{g_{\boldsymbol{\delta}}}
\newcommand{\pgdel}{\pdg{g}_{\boldsymbol{\delta}}}
\newcommand{\bmz}{\bar{M}_z}
\newcommand{\calbmx}{{\cal \bar{M}}_x}
\newcommand{\calgdel}{\pdg{\breve{g}}_{\sma{\bdelta}}}
\newcommand{\brevegdel}{\pdg{\breve{g}}_{\sma{\bdelta}}}
\newcommand{\brevebmx}{\breve{\bar{M}}_x}
\newcommand{\uit}{U_{\sma{\cali T}}}
\newcommand{\utg}{U_{\sma{Tg \bdelta}}}
\newcommand{\ut}{U_{\sma{T}}}
\newcommand{\ug}{U_{\sma{g \bdelta}}}
\newcommand{\ubmx}{U_{\sma{\bmx}}}
\newcommand{\utbmz}{U_{\sma{T\bmz}}}
\newcommand{\calug}{\calg_{\sma{\bdelta}}}
\newcommand{\caluit}{\calu_{\sma{\cali T}}}
\newcommand{\caltgdel}{\breve{T}_{\sma{g \bdelta}}}
\newcommand{\brevetgdel}{\breve{T}_{\sma{g \bdelta}}}
\newcommand{\brevetbmx}{\breve{T}_{\sma{\bmx}}}
\newcommand{\hattbmx}{\hat{T}_{\sma{\bmx}}}
\newcommand{\brevetbmz}{\breve{T}_{\sma{\bmz}}}
\newcommand{\breveti}{\breve{T}_{\sma{\cali}}}
\newcommand{\caltbmz}{\calt_{\sma{\bmz}}}
\newcommand{\caltbmx}{\calt_{\sma{\bmx}}}
\newcommand{\calut}{\calu_{\sma{T}}}
\newcommand{\hatgdel}{\pdg{\hat{g}}_{\sma{\bdelta}}}
\newcommand{\hatTg}{\pdg{\hat{T}}_{\sma{g\bdelta}}}
\newcommand\csixdel{C_{\sma{6,\bdelta}}}
\newcommand\brevecsixdel{\breve{C}_{\sma{6,\bdelta}}}
\newcommand\cthreedel{C_{\sma{3,\bdelta}}}
\newcommand\brevecthreedel{\breve{C}_{\sma{3,\bdelta}}}
\newcommand\hatcthreedel{\hat{C}_{\sma{3,\bdelta}}}
\newcommand\cthreetwodel{C_{\sma{3,2\bdelta}}}
\newcommand\brevecthreetwodel{\breve{C}_{\sma{3,2\bdelta}}}
\newcommand\brevectwothreedel{\breve{C}_{\sma{2,3\bdelta}}}
\newcommand\ctwothreedel{C_{\sma{2,3\bdelta}}}
\newcommand\hatcsixdel{\hat{C}_{\sma{6,\bdelta}}}
\newcommand\ucsixdel{U_{\sma{C_6,\bdelta}}}
\newcommand\cndel{C_{\sma{n,\bdelta}}}
\newcommand\cbarndel{C_{\sma{\bar{n},\bdelta}}}
\newcommand\ucndel{U_{\sma{C_n,\bdelta}}}
\newcommand\hatcndel{\hat{C}_{\sma{n,\bdelta}}}
\newcommand\brevecndel{\breve{C}_{\sma{n,\bdelta}}}
\newcommand\brevectwotwodel{\breve{C}_{\sma{2,2\bdelta}}}
\newcommand\brevecfourdel{\breve{C}_{\sma{4,\bdelta}}}
\newcommand\brevectwodel{\breve{C}_{\sma{2,\bdelta}}}


% vectors and matrices
\newcommand{\vectwo}[2]{\begin{pmatrix} {#1}\\{#2} \end{pmatrix}}
\newcommand{\matrixtwo}[4]{\begin{pmatrix} #1 & #2 \\ #3 & #4 \end{pmatrix}}
\newcommand{\diagmatrix}[2]{\begin{pmatrix} #1 & 0 \\ 0 & #2 \end{pmatrix}}
\newcommand{\matrixthree}[9]{\begin{pmatrix} #1 & #2 & #3 \\ #4 & #5 & #6 \\ #7 & #8 & #9 \end{pmatrix}}


% Pauli matrices
\newcommand{\szero}{\sigma_{\sma{0}}}
\newcommand{\sx}{\sigma_{\sma{1}}}
\newcommand{\sy}{\sigma_{\sma{2}}}
\newcommand{\sz}{\sigma_{\sma{3}}}
\newcommand{\tzero}{\tau_{\sma{0}}}
\newcommand{\tx}{\tau_{\sma{1}}}
\newcommand{\ty}{\tau_{\sma{2}}}
\newcommand{\tz}{\tau_{\sma{3}}}



% parafermion operators
\newcommand{\gt}{\gamma_{\sma{2}}}
\newcommand{\gth}{\gamma_{\sma{3}}}
\newcommand{\gfo}{\gamma_{\sma{4}}}
\newcommand{\gfi}{\gamma_{\sma{5}}}
\newcommand{\gj}{\gamma_{\sma{j}}}
\newcommand{\gtj}{\gamma_{\sma{2j}}}
\newcommand{\gtjpo}{\gamma_{\sma{2j+1}}}
\newcommand{\gtjpt}{\gamma_{\sma{2j+2}}}
\newcommand{\gtjmo}{\gamma_{\sma{2j-1}}}
\newcommand{\gtL}{\gamma_{\sma{2L}}}
\newcommand{\gtLpo}{\gamma_{\sma{2L+1}}}
\newcommand{\gtLpt}{\gamma_{\sma{2L+2}}}
\newcommand{\gtLmo}{\gamma_{\sma{2L-1}}}
\newcommand{\gtLmt}{\gamma_{\sma{2L-2}}}
\newcommand{\gtLmth}{\gamma_{\sma{2L-3}}}
\newcommand{\gtLmfo}{\gamma_{\sma{2L-4}}}


% insert text in equation
\newcommand{\ins}[1]{\;\;\;\;\text{#1}\;\;\;\;}


%momentum parallel and perpendicular
\newcommand{\kpar}{\boldsymbol{k}_{{\shortparallel}}}
\newcommand{\Dpar}{D^{g}_{{\shortparallel}}}
\newcommand{\kper}{k_{\perp}}


% Cnv 
\newcommand{\ctv}{C_{3v}}
\newcommand{\cfv}{C_{4v}}
\newcommand{\csv}{C_{6v}}
\newcommand{\cnv}{C_{nv}}


%C_n Time-reversal
\newcommand{\cnt}{C_n {\cal T}}
\newcommand{\cn}{C_n}
\newcommand{\cfour}{C_4}
\newcommand{\cs}{C_6}
\newcommand{\ct}{C_3}
\newcommand{\cst}{C_6{\cal T}}
\newcommand{\cft}{C_4{\cal T}}
\newcommand{\ctt}{C_2{\cal T}}


% average 
\newcommand{\ave}[1]{\langle\,#1\,\rangle}



%inverse Angstroms and Angstroms
\newcommand{\invA}{\mathrm{\AA^{\scriptscriptstyle{-1}}}}
\newcommand{\ang}{\mathrm{\AA}}

% Lagrangian
\newcommand{\lag}{{\mathscr{L}}}


% green's function
\newcommand{\green}{{\mathscr{G}}}

% Cauchy principal value
\newcommand{\prin}{{\mathscr{P}}}

% imaginary and real parts
\newcommand{\imag}{{\mathscr{I}}}
\newcommand{\real}{{\mathscr{R}}}


%total differentiation
\newcommand{\totaldif}[2]{\frac{ d #1}{d #2}}

% calligraphic font
\newcommand{\cala}{{\cal A}}
\newcommand{\calb}{{\cal B}}
\newcommand{\calc}{{\cal C}}
\newcommand{\cald}{{\cal D}}
\newcommand{\cale}{{\cal E}}
\newcommand{\calf}{{\cal F}}
\newcommand{\calg}{{\cal G}}
\newcommand{\calh}{{\cal H}}
\newcommand{\tcalh}{\tilde{\cal H}}
\newcommand{\cali}{{\cal I}}
\newcommand{\calj}{{\cal J}}
\newcommand{\calk}{{\cal K}}
\newcommand{\call}{{\cal L}}
\newcommand{\calm}{{\cal M}}
\newcommand{\caln}{{\cal N}}
\newcommand{\calo}{{\cal O}}
\newcommand{\calp}{{\cal P}}
\newcommand{\calq}{{\cal Q}}
\newcommand{\calr}{{\cal R}}
\newcommand{\cals}{{\cal S}}
\newcommand{\calt}{{\cal T}}
\newcommand{\calu}{{\cal U}}
\newcommand{\calv}{{\cal V}}
\newcommand{\calw}{{\cal W}}
\newcommand{\calx}{{\cal X}}
\newcommand{\caly}{{\cal Y}}
\newcommand{\calz}{{\cal Z}}

% mathscript font
\newcommand{\scra}{{\mathscr A}}
\newcommand{\scrb}{{\mathscr B}}
\newcommand{\scrc}{{\mathscr C}}
\newcommand{\scrd}{{\mathscr D}}
\newcommand{\scre}{{\mathscr E}}
\newcommand{\barscre}{\bar{\mathscr E}}
\newcommand{\scrf}{{\mathscr F}}
\newcommand{\scrg}{{\mathscr G}}
\newcommand{\scrh}{{\mathscr H}}
\newcommand{\tscrh}{\tilde{\mathscr H}}
\newcommand{\scri}{{\mathscr I}}
\newcommand{\scrj}{{\mathscr J}}
\newcommand{\scrk}{{\mathscr K}}
\newcommand{\scrl}{{\mathscr L}}
\newcommand{\scrm}{{\mathscr M}}
\newcommand{\scrn}{{\mathscr N}}
\newcommand{\scro}{{\mathscr O}}
\newcommand{\scrp}{{\mathscr P}}
\newcommand{\scrq}{{\mathscr Q}}
\newcommand{\scrr}{{\mathscr R}}
\newcommand{\scrs}{{\mathscr S}}
\newcommand{\scrt}{{\mathscr T}}
\newcommand{\scru}{{\mathscr U}}
\newcommand{\scrv}{{\mathscr V}}
\newcommand{\scrw}{{\mathscr W}}
\newcommand{\scrx}{{\mathscr X}}
\newcommand{\scry}{{\mathscr Y}}
\newcommand{\scrz}{{\mathscr Z}}


%Gamma matrices
\newcommand{\gam}[1]{\Gamma_{#1}}

%determinant
\newcommand{\de}[1]{\text{det}[\;#1\;]}

%trace
\newcommand{\tr}{\text{Tr}}




\newcommand{\noi}[1]{\noindent (#1)}
\newcommand{\imp}{\;\;\Rightarrow\;\;}
\newcommand{\mo}{\text{-}1}
\newcommand{\mt}{\text{-}2}
\newcommand{\minus}{\text{-}}
\newcommand{\oneover}[1]{\tfrac{1}{#1}}


% A command for inner product and bras and kets
\newcommand{\braket}[2]{\big\langle #1 \big| #2 \big\rangle}
\newcommand{\ketbra}[2]{\big|  #1  \big\rangle \big\langle #2 \big| }
\newcommand{\braopket}[3]{\big\langle #1 \big| #2 \big| #3 \big\rangle}
\newcommand{\bra}[1]{\big\langle#1\big|}
\newcommand{\ket}[1]{\big|#1\big\rangle}
\newcommand{\bigket}[1]{\bigl|#1\bigr\rangle}
\newcommand{\textket}[1]{|#1\rangle}
  %double bras and kets
	\newcommand{\dbraket}[2]{\big\langle\big\langle #1 \big| #2 \big\rangle \big\rangle}
  \newcommand{\dketbra}[2]{\big|  #1  \big\rangle\big\rangle \big\langle \big\langle #2 \big| }
  \newcommand{\dbraopket}[3]{\big\langle \big\langle #1 \big| #2 \big| #3 \big\rangle \big\rangle}
  \newcommand{\dket}[1]{\big|#1\big\rangle \big\rangle}
  \newcommand{\dbra}[1]{\big\langle \big\langle#1\big|}
  \newcommand{\dexp}[1]{\big\langle\big\langle #1 \big\rangle \big\rangle}



% Various bracketing commands
\newcommand{\of}[1]{\!\left(#1\right)}
\newcommand{\sqof}[1]{\left[#1\right]}
\newcommand{\cuof}[1]{\left\{#1\right\}}

% commutator and anticommutator
\newcommand{\comm}[2]{\left[#1,#2\right]}
\newcommand{\anticomm}[2]{\left\{#1,#2\right\}}
% sum on nearest neighbor bonds
\newcommand{\bond}{\left\langle i, j \right\rangle}
%\newcommand{\bondsum}{\sum_{\left\langle i, j \right\rangle}}
\newcommand{\nbond}{\left\langle\left\langle i, j \right\rangle\right\rangle}
% 1/2
\newcommand{\half}{\frac{1}{2} }
\newcommand{\thalf}{\tfrac{1}{2} }
% simplifies using the up and down arrows to denote spin
\newcommand{\up}{\uparrow}
\newcommand{\down}{\downarrow}
% Absolute value  
\newcommand{\abs}[1]{\left|#1\right|}

% Roman functions for real and imaginary parts
\newcommand{\re}{\mathrm{Re}}
\newcommand{\im}{\mathrm{Im}}


%Expectation values
\newcommand{\expect}[1]{\left\langle#1\right\rangle}
\newcommand{\pdag}{\phantom{\dagger}}
\newcommand{\pdg}[1]{{#1}^{\phantom{\dagger}}}

\newcommand{\bkap}{\bar{\glide}}
\newcommand{\bchi}{\bar{\chi}}
\newcommand{\baeta}{\bar{\eta}}
\newcommand{\lin}{\notag \\}



\newcommand{\ab}{\alpha\beta}
\newcommand{\deli}{\Delta^{-1}}


\newcommand{\ra}{{R\,\alpha}}
\newcommand{\rax}{{R+\vec{x}\,\alpha}}

\newcommand{\rb}{{R'\,\beta}}
\newcommand{\rarb}{{R\,\alpha};R'\,\beta}
\newcommand{\zth}{\mathbb{Z}_3}


\newcommand{\xin}{x_{\tex{inv}}}
\newcommand{\low}{L$\ddot{\text{o}}$wdin\;}
\newcommand{\tex}[1]{\sma{\text{#1}}}











\newcommand{\kf}{k_{\scriptscriptstyle{F}}}

\newcommand{\bfk}{\boldsymbol{k}}
\newcommand{\bfq}{\boldsymbol{q}}



\newcommand{\bpm}{\begin{pmatrix}}
\newcommand{\epm}{\end{pmatrix}}
\newcommand{\nk}{n_{\boldsymbol{k}'}}
\newcommand{\dk}{\Delta_{\boldsymbol{k}'}}
\newcommand{\Dk}{\Delta_{\boldsymbol{k}}}
\newcommand{\tk}{\tilde{k}}
\newcommand{\tkp}{\tilde{k}'}
\newcommand{\bal}{\begin{align}}
\newcommand{\Ainv}{\mathrm{\AA^{\scriptscriptstyle{-1}}}}

\newcommand{\V}{V_{\text{eff}}}
\newcommand{\si}{\;\text{sin}\,}
\newcommand{\ta}{\;\text{tan}\,}
\newcommand{\co}{\;\text{\text{cos}}\,}
\newcommand{\te}{t_{\text{eff}}}
\newcommand{\ep}{\bar{\epsilon}}



\newcommand{\braa}[1]{\left\langle#1\right|_{\scriptscriptstyle{A}}}
\newcommand{\brab}[1]{\left\langle#1\right|_{\scriptscriptstyle{B}}}

\newcommand{\dg}[1]{#1^{\scriptstyle{\dagger}}}
\newcommand{\bof}[1]{\boldsymbol{#1}}
\newcommand{\sma}[1]{\scriptscriptstyle{#1}}
\newcommand{\po}{{\sma{+}} 1}



\newcommand{\noc}{n_{\sma{{occ}}}}
\newcommand{\ntot}{n_{\sma{{tot}}}}

\newtheorem{definition}{Definition}[section]
